HingePlace: Harnessing the neural thresholding behavior to optimize Transcranial Electrical Stimulation

Transcranial Electrical Stimulation (tES) is a neuromodulation technique that utilizes electrodes on the scalp to stimulate target brain regions. tES has shown promise in treating many neurological conditions, such as stroke rehabilitation and chronic pain. Several electrode placement algorithms have been proposed to optimize tES-based therapies by designing multi-electrode montages that create focal neural responses. We first extend a well-known unification result by Fernandez-Corazza et al. to unify all major traditional electrode placement algorithms. We utilize this unification result to identify a common restriction among traditional electrode placement algorithms: they do not harness the thresholding behavior of neural response. Consequently, these algorithms only partially harness the properties of neural response to optimize tES, particularly increasing the focality of neural response. We propose a new electrode placement algorithm, HingePlace, that utilizes a symmetrized hinge loss to harness the thresholding behavior of neural response. We extensively compare the HingePlace algorithm with traditional electrode placement algorithms in two simulation platforms. Across both platforms, we find that HingePlace-designed montages consistently generate more focal neural responses -- by as much as 60% -- than the electrode montages designed by traditional electrode placement algorithms.

==> references.tex <==
\begin{thebibliography}{10}

\bibitem{kalu2012transcranial}
UG~Kalu, CE~Sexton, CK~Loo, and KP~Ebmeier.
\newblock Transcranial direct current stimulation in the treatment of major depression: a meta-analysis.
\newblock {\em Psychological medicine}, 42(9):1791, 2012.

\bibitem{mori2010effects}
Francesco Mori, Claudia Codec{\`a}, Hajime Kusayanagi, Fabrizia Monteleone, Fabio Buttari, Stefania Fiore, Giorgio Bernardi, Giacomo Koch, and Diego Centonze.
\newblock Effects of anodal transcranial direct current stimulation on chronic neuropathic pain in patients with multiple sclerosis.
\newblock {\em The Journal of Pain}, 11(5):436--442, 2010.

\bibitem{yook2011suppression}
Soon-Won Yook, Sung-Hee Park, Jeong-Hwan Seo, Sun-Jun Kim, and Myoung-Hwan Ko.
\newblock Suppression of seizure by cathodal transcranial direct current stimulation in an epileptic patient-a case report.
\newblock {\em Annals of rehabilitation medicine}, 35(4):579--582, 2011.

\bibitem{brunoni2013transcranial}
Andre~R Brunoni, Felipe Fregni, Alberto Priori, Roberta Ferrucci, and Paulo~S{\'e}rgio Boggio.
\newblock Transcranial direct current stimulation: challenges, opportunities, and impact on psychiatry and neurorehabilitation.
\newblock {\em Frontiers in psychiatry}, 4:19, 2013.

\bibitem{parkin2015non}
Beth~L Parkin, Hamed Ekhtiari, and Vincent~F Walsh.
\newblock Non-invasive human brain stimulation in cognitive neuroscience: a primer.
\newblock {\em Neuron}, 87(5):932--945, 2015.

\bibitem{kuo2013comparing}
Hsiao-I Kuo, Marom Bikson, Abhishek Datta, Preet Minhas, Walter Paulus, Min-Fang Kuo, and Michael~A Nitsche.
\newblock Comparing cortical plasticity induced by conventional and high-definition 4$\times$ 1 ring tdcs: a neurophysiological study.
\newblock {\em Brain stimulation}, 6(4):644--648, 2013.

\bibitem{fischer2017multifocal}
David~B Fischer, Peter~J Fried, Giulio Ruffini, Oscar Ripolles, Ricardo Salvador, Jaume Banus, William~Tyler Ketchabaw, Emiliano Santarnecchi, Alvaro Pascual-Leone, and Michael~D Fox.
\newblock Multifocal tdcs targeting the resting state motor network increases cortical excitability beyond traditional tdcs targeting unilateral motor cortex.
\newblock {\em Neuroimage}, 157:34--44, 2017.

\bibitem{dmochowski2011optimized}
Jacek~P. Dmochowski, Abhishek Dutta, Marom Bikson, Yuzhuo Su, and Lucas~C. Parra.
\newblock Optimized multi-electrode stimulation increases focality and intensity at target.
\newblock {\em Journal of Neural Engineering}, 8(4):046011, 2011.

\bibitem{horvath2014transcranial}
Jared~C Horvath, Olivia Carter, and Jason~D Forte.
\newblock Transcranial direct current stimulation: five important issues we aren't discussing (but probably should be).
\newblock {\em Frontiers in systems neuroscience}, 8:2, 2014.

\bibitem{horvath2015evidence}
Jared~Cooney Horvath, Jason~D Forte, and Olivia Carter.
\newblock Evidence that transcranial direct current stimulation (tdcs) generates little-to-no reliable neurophysiologic effect beyond mep amplitude modulation in healthy human subjects: a systematic review.
\newblock {\em Neuropsychologia}, 66:213--236, 2015.

\bibitem{antal2015conceptual}
A~Antal, D~Keeser, A~Priori, F~Padberg, and MA~Nitsche.
\newblock Conceptual and procedural shortcomings of the systematic review “evidence that transcranial direct current stimulation (tdcs) generates little-to-no reliable neurophysiologic effect beyond mep amplitude modulation in healthy human subjects: a systematic review” by horvath and co-workers.
\newblock {\em Brain Stimulation: Basic, Translational, and Clinical Research in Neuromodulation}, 8(4):846--849, 2015.

\bibitem{laakso2019can}
Ilkka Laakso, Marko Mikkonen, Soichiro Koyama, Akimasa Hirata, and Satoshi Tanaka.
\newblock Can electric fields explain inter-individual variability in transcranial direct current stimulation of the motor cortex?
\newblock {\em Scientific reports}, 9(1):626, 2019.

\bibitem{fernandez2020unification}
Mariano Fernández-Corazza, Sergei Turovets, and Carlos~Horacio Muravchik.
\newblock Unification of optimal targeting methods in transcranial electrical stimulation.
\newblock {\em NeuroImage}, 209:116403, 2020.

\bibitem{im2008determination}
Chang-Hwan Im, Hui-Hun Jung, Jung-Do Choi, Soo~Yeol Lee, and Ki-Young Jung.
\newblock Determination of optimal electrode positions for transcranial direct current stimulation ({tDCS}).
\newblock {\em Physics in Medicine \& Biology}, 53(11):N219, 2008.

\bibitem{park2011novel}
Ji-Hye Park, Seung~Bong Hong, Do-Won Kim, Minah Suh, and Chang-Hwan Im.
\newblock A novel array-type transcranial direct current stimulation (tdcs) system for accurate focusing on targeted brain areas.
\newblock {\em IEEE Transactions on Magnetics}, 47(5):882--885, 2011.

\bibitem{sadleir2012target}
Rosalind Sadleir, Tracy~D. Vannorsdall, David~J. Schretlen, and Barry Gordon.
\newblock Target optimization in transcranial direct current stimulation.
\newblock {\em Frontiers in Psychiatry}, 3, 2012.

\bibitem{dutta2013using}
Arindam Dutta and Anirban Dutta.
\newblock Using electromagnetic reciprocity and magnetic resonance current density imaging to fit multi-electrode montage for non-invasive brain stimulation.
\newblock In {\em 2013 6th International IEEE/EMBS Conference on Neural Engineering (NER)}, pages 447--451. IEEE, 2013.

\bibitem{ruffini2014optimization}
Giulio Ruffini, Michael~D. Fox, Oscar Ripolles, Pedro Cavaleiro~Miranda, and Alvaro Pascual-Leone.
\newblock Optimization of multifocal transcranial current stimulation for weighted cortical pattern targeting from realistic modeling of electric fields.
\newblock {\em NeuroImage}, 89:216--225, 2014.

\bibitem{guler2016optimization}
Seyhmus Guler, Moritz Dannhauer, Burak Erem, Rob Macleod, Don Tucker, Sergei Turovets, Phan Luu, Deniz Erdogmus, and Dana~H. Brooks.
\newblock Optimization of focality and direction in dense electrode array transcranial direct current stimulation {(tDCS)}.
\newblock {\em Journal of Neural Engineering}, 13(3):036020, May 2016.

\bibitem{salman2016concurrency}
Adnan Salman, Allen Malony, Sergei Turovets, Vasily Volkov, David Ozog, and Don Tucker.
\newblock Concurrency in electrical neuroinformatics: parallel computation for studying the volume conduction of brain electrical fields in human head tissues.
\newblock {\em Concurrency and Computation: Practice and Experience}, 28(7):2213--2236, 2016.

\bibitem{cancelli2016simple}
Andrea Cancelli, Carlo Cottone, Franca Tecchio, Dennis~Q Truong, Jacek Dmochowski, and Marom Bikson.
\newblock A simple method for {EEG} guided transcranial electrical stimulation without models.
\newblock {\em Journal of neural engineering}, 13(3):036022, 2016.

\bibitem{wagner2016optimization}
Sven Wagner, Martin Burger, and Carsten~H. Wolters.
\newblock An optimization approach for well-targeted transcranial direct current stimulation.
\newblock {\em SIAM Journal on Applied Mathematics}, 76(6):2154--2174, 2016.

\bibitem{fernandez2016transcranial}
Mariano Fernández-Corazza, Sergei Turovets, Phan Luu, Erik Anderson, and Don Tucker.
\newblock Transcranial electrical neuromodulation based on the reciprocity principle.
\newblock {\em Frontiers in Psychiatry}, 7, 2016.

\bibitem{dmochowski2017optimal}
Jacek~P Dmochowski, Laurent Koessler, Anthony~M Norcia, Marom Bikson, and Lucas~C Parra.
\newblock Optimal use of eeg recordings to target active brain areas with transcranial electrical stimulation.
\newblock {\em Neuroimage}, 157:69--80, 2017.

\bibitem{guler2018computationally}
Seyhmus Guler, Moritz Dannhauer, Biel Roig-Solvas, Alexis Gkogkidis, Rob Macleod, Tonio Ball, Jeffrey~G Ojemann, and Dana~H Brooks.
\newblock Computationally optimized {ECoG} stimulation with local safety constraints.
\newblock {\em Neuroimage}, 173:35--48, 2018.

\bibitem{saturnino2019accessibility}
Guilherme~Bicalho Saturnino, Hartwig~Roman Siebner, Axel Thielscher, and Kristoffer~Hougaard Madsen.
\newblock Accessibility of cortical regions to focal tes: Dependence on spatial position, safety, and practical constraints.
\newblock {\em NeuroImage}, 203:116183, 2019.

\bibitem{khan2022individually}
Asad Khan, Marios Antonakakis, Nikolas Vogenauer, Jens Haueisen, and Carsten~H. Wolters.
\newblock Individually optimized multi-channel {tDCS} for targeting somatosensory cortex.
\newblock {\em Clinical Neurophysiology}, 134:9--26, 2022.

\bibitem{prieto2022l1}
Fernando {Galaz Prieto}, Atena Rezaei, Maryam Samavaki, and Sampsa Pursiainen.
\newblock L1-norm vs. l2-norm fitting in optimizing focal multi-channel {tES} stimulation: linear and semidefinite programming vs. weighted least squares.
\newblock {\em Computer Methods and Programs in Biomedicine}, 226:107084, 2022.

\bibitem{wang2023multi}
Mo~Wang, Kexin Lou, Zeming Liu, Pengfei Wei, and Quanying Liu.
\newblock Multi-objective optimization via evolutionary algorithm (movea) for high-definition transcranial electrical stimulation of the human brain.
\newblock {\em NeuroImage}, 280:120331, 2023.

\bibitem{kandel2000principles}
Eric~R Kandel, James~H Schwartz, Thomas~M Jessell, Steven Siegelbaum, A~James Hudspeth, and Sarah Mack.
\newblock {\em Principles of neural science}, volume~4.
\newblock McGraw-hill New York, 2000.

\bibitem{hsu2023robust}
Gavin Hsu, A~Duke Shereen, Leonardo~G Cohen, and Lucas~C Parra.
\newblock Robust enhancement of motor sequence learning with 4 ma transcranial electric stimulation.
\newblock {\em Brain stimulation}, 16(1):56--67, 2023.

\bibitem{huang2019realistic}
Yu~Huang, Abhishek Datta, Marom Bikson, and Lucas~C Parra.
\newblock Realistic volumetric-approach to simulate transcranial electric stimulation—roast—a fully automated open-source pipeline.
\newblock {\em Journal of neural engineering}, 16(5):056006, 2019.

\bibitem{Caldas-Martinez2024}
Sara Caldas-Martinez, Chaitanya Goswami, Mats Forssell, Jiaming Cao, Alison~L. Barth, and Pulkit Grover.
\newblock Cell-specific effects of temporal interference stimulation on cortical function.
\newblock {\em Communications Biology}, 7(1):1076, Sep 2024.

\bibitem{griffiths2005introduction}
David~J Griffiths.
\newblock Introduction to electrodynamics, 2005.

\bibitem{goswami2021hingeplace}
Chaitanya Goswami and Pulkit Grover.
\newblock Hingeplace: Focused transcranial electrical current stimulation that allows subthreshold fields outside the stimulation target.
\newblock In {\em 2021 43rd Annual International Conference of the IEEE Engineering in Medicine \& Biology Society (EMBC)}, pages 1577--1583, 2021.

\bibitem{gomez2024perspectives}
Jose Gomez-Tames and Mariano Fern{á}ndez-Corazza.
\newblock Perspectives on optimized transcranial electrical stimulation based on spatial electric field modeling in humans.
\newblock {\em Journal of Clinical Medicine}, 13(11), 2024.

\bibitem{aberra2018biophysically}
Aman~S Aberra, Angel~V Peterchev, and Warren~M Grill.
\newblock Biophysically realistic neuron models for simulation of cortical stimulation.
\newblock {\em Journal of neural engineering}, 15(6):066023, 2018.

\bibitem{rattay1986analysis}
Frank Rattay.
\newblock Analysis of models for external stimulation of axons.
\newblock {\em IEEE Transactions on Biomedical Engineering}, BME-33(10):974--977, 1986.

\bibitem{rattay1999basic}
Frank Rattay.
\newblock The basic mechanism for the electrical stimulation of the nervous system.
\newblock {\em Neuroscience}, 89(2):335--346, 1999.

\bibitem{fellner2022finite}
Andreas Fellner, Amirreza Heshmat, Paul Werginz, and Frank Rattay.
\newblock A finite element method framework to model extracellular neural stimulation.
\newblock {\em Journal of Neural Engineering}, 19(2):022001, 2022.

\bibitem{Hermann2020}
Bertrand Hermann, Federico Raimondo, Lukas Hirsch, Yu~Huang, M{\'e}lanie Denis-Valente, Pauline P{\'e}rez, Denis Engemann, Fr{\'e}d{\'e}ric Faugeras, Nicolas Weiss, Sophie Demeret, Benjamin Rohaut, Lucas~C. Parra, Jacobo~D. Sitt, and Lionel Naccache.
\newblock Combined behavioral and electrophysiological evidence for a direct cortical effect of prefrontal tdcs on disorders of consciousness.
\newblock {\em Scientific Reports}, 10(1):4323, Mar 2020.

\bibitem{farahani2024transcranial}
Forouzan Farahani, Niranjan Khadka, Lucas~C Parra, Marom Bikson, and Mih{\'a}ly V{\"o}r{\"o}slakos.
\newblock Transcranial electric stimulation modulates firing rate at clinically relevant intensities.
\newblock {\em Brain Stimulation}, 17(3):561--571, 2024.

\bibitem{forssellner2021}
Mats Forssell, Vishal Jain, Chaitanya Goswami, Sara Caldas-Martinez, Pulkit Grover, and Maysam Chamanzar.
\newblock Effect of focality of transcranial currents on neural responses.
\newblock In {\em 2021 10th International IEEE/EMBS Conference on Neural Engineering (NER)}, pages 289--292, 2021.

\bibitem{ayache2012stroke}
Samar~S Ayache, Wassim~H Farhat, Hela~G Zouari, Hassan Hosseini, Veit Mylius, and Jean-Pascal Lefaucheur.
\newblock Stroke rehabilitation using noninvasive cortical stimulation: motor deficit.
\newblock {\em Expert review of neurotherapeutics}, 12(8):949--972, 2012.

\bibitem{sun2022repetitive}
Pingping Sun, Lei Fang, Jianzhong Zhang, Yang Liu, Guodong Wang, and Rui Qi.
\newblock Repetitive transcranial magnetic stimulation for patients with fibromyalgia: a systematic review with meta-analysis.
\newblock {\em Pain Medicine}, 23(3):499--514, 2022.

\bibitem{szelenyi2007transcranial}
Andrea Szel{\'e}nyi, Karl~F Kothbauer, and Vedran Deletis.
\newblock Transcranial electric stimulation for intraoperative motor evoked potential monitoring: stimulation parameters and electrode montages.
\newblock {\em Clinical neurophysiology}, 118(7):1586--1595, 2007.

\bibitem{alam2016spatial}
Mahtab Alam, Dennis~Q Truong, Niranjan Khadka, and Marom Bikson.
\newblock Spatial and polarity precision of concentric high-definition transcranial direct current stimulation (hd-tdcs).
\newblock {\em Physics in Medicine \& Biology}, 61(12):4506, 2016.

\bibitem{miranda2014predicting}
Pedro~C Miranda, Abeye Mekonnen, Ricardo Salvador, and Peter~J Basser.
\newblock Predicting the electric field distribution in the brain for the treatment of glioblastoma.
\newblock {\em Physics in Medicine \& Biology}, 59(15):4137, 2014.

\bibitem{boyd2004convex}
Stephen Boyd, Stephen~P Boyd, and Lieven Vandenberghe.
\newblock {\em Convex optimization}.
\newblock Cambridge university press, 2004.

\bibitem{gorski2007biconvex}
Jochen Gorski, Frank Pfeuffer, and Kathrin Klamroth.
\newblock Biconvex sets and optimization with biconvex functions: a survey and extensions.
\newblock {\em Mathematical methods of operations research}, 66(3):373--407, 2007.

\bibitem{hiriart1996convex}
Jean-Baptiste Hiriart-Urruty and Claude Lemar{\'e}chal.
\newblock {\em Convex analysis and minimization algorithms I: Fundamentals}, volume 305.
\newblock Springer science \& business media, 1996.

\bibitem{bertsekas2009convex}
Dimitri Bertsekas.
\newblock {\em Convex optimization theory}, volume~1.
\newblock Athena Scientific, 2009.

\bibitem{oostenveld2001five}
Robert Oostenveld and Peter Praamstra.
\newblock The five percent electrode system for high-resolution eeg and erp measurements.
\newblock {\em Clinical neurophysiology}, 112(4):713--719, 2001.

\bibitem{forssell2021effect}
Mats Forssell, Chaitanya Goswami, Ashwati Krishnan, Maysamreza Chamanzar, and Pulkit Grover.
\newblock Effect of skull thickness and conductivity on current propagation for noninvasively injected currents.
\newblock {\em Journal of Neural Engineering}, 2021.

\bibitem{markram2015reconstruction}
Henry Markram, Eilif Muller, Srikanth Ramaswamy, Michael~W Reimann, Marwan Abdellah, Carlos~Aguado Sanchez, Anastasia Ailamaki, Lidia Alonso-Nanclares, Nicolas Antille, Selim Arsever, et~al.
\newblock Reconstruction and simulation of neocortical microcircuitry.
\newblock {\em Cell}, 163(2):456--492, 2015.

\bibitem{carnevale2006neuron}
Nicholas~T Carnevale and Michael~L Hines.
\newblock The neuron book, 2006.

\bibitem{hines2009neuron}
Michael Hines, Andrew~P Davison, and Eilif Muller.
\newblock Neuron and python.
\newblock {\em Frontiers in neuroinformatics}, 3:391, 2009.

\bibitem{merton1980stimulation}
PA~Merton and HB~Morton.
\newblock Stimulation of the cerebral cortex in the intact human subject.
\newblock {\em Nature}, 285(5762):227--227, 1980.

\bibitem{diamond2016cvxpy}
Steven Diamond and Stephen Boyd.
\newblock {CVXPY}: {A} {P}ython-embedded modeling language for convex optimization.
\newblock {\em Journal of Machine Learning Research}, 17(83):1--5, 2016.

\bibitem{agrawal2018rewriting}
Akshay Agrawal, Robin Verschueren, Steven Diamond, and Stephen Boyd.
\newblock A rewriting system for convex optimization problems.
\newblock {\em Journal of Control and Decision}, 5(1):42--60, 2018.

\bibitem{10.5555/1593511}
Guido Van~Rossum and Fred~L. Drake.
\newblock Python 3 reference manual, 2009.

\bibitem{costa2021further}
Luciano da~F Costa.
\newblock Further generalizations of the jaccard index.
\newblock {\em arXiv preprint arXiv:2110.09619}, 2021.

\end{thebibliography}

